Cyber physical modeling of distributed resources for distribution system operations

Co-simulation platforms are necessary to study the interactions of complex systems integrated in future smart grids. The Virtual Grid Integration Laboratory (VirGIL) is a modular co-simulation platform designed to study interactions between demand response strategies, building comfort, communication networks, and power system operation. This paper presents the coupling of power systems, buildings, communications and control under a master algorithm. There are two objectives. First, to use a modular architecture for VirGIL, based on the Functional Mock-up Interface (FMI), where several different modules can be added, exchanged, and tested. Second, to use a commercial power system simulation platform, familiar to power system operators, such as DIgSILENT Powerfactory. This will help reduce the barriers to the industry for adopting such platforms, investigate and subsequently deploy demand response strategies in their daily operation. VirGIL further introduces the integration of the Quantized State System (QSS) methods for simulation in this co-simulation platform. Results on how these systems interact using a real network and consumption data are also presented.

==> Makefile <==
LaTeX=IEEE_Proceedings


all: compile clean open

preprint: compile-preprint clean

compile:
	pdflatex $(LaTeX).tex
	pdflatex $(LaTeX).tex
	bibtex $(LaTeX).aux
	pdflatex $(LaTeX).tex
	pdflatex $(LaTeX).tex

clean:
	find . -name \*~    | xargs rm -f
	find . -name \*.glo | xargs rm -f
	find . -name \*.nlo | xargs rm -f
	find . -name \*.spl | xargs rm -f 
	find . -name \*.log | xargs rm -f 
	find . -name \*.lot | xargs rm -f 
	find . -name \*.toc | xargs rm -f 
	find . -name \*.out | xargs rm -f 
	find . -name \*.blg | xargs rm -f 
	find . -name \*.aux | xargs rm -f 
	find . -name \*.ps  | xargs rm -f 
	find . -name \*.dvi | xargs rm -f 
	find . -name \*.snm | xargs rm -f 
	find . -name \*.vrb | xargs rm -f 
	find . -name \*.nav | xargs rm -f

view:
	open *.pdf


==> text/case_IEEE.tex <==
\subsection{IEEE case ???}
\label{sec:case_IEEE}

\textbf{??}

\begin{itemize}
\item Possibly a more complicated IEEE Test System
\end{itemize}

==> text/simulation_building.tex <==
\begin{itemize}
\item Transform the diagram in the picture to a figure and provide a description.
\item Provide a figure and details how the building itself is modeled.
\end{itemize}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1\linewidth]{figures/Building_DR_State_Diagram}
    \caption{State Diagram for the Demand Response Signals to the Buildings.}
    \label{fig:Building_DR_State_Diagram}%\vspace{-0.3cm}
\end{figure}


==> text/simulation_intro.tex <==
What is our simulation setup. Who interacts with whom. What information is being exchanged, at what time scales, etc. Transform the following picture in a figure and describe it.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1\linewidth]{figures/ISO_DR_Interactions}
    \caption{Interactions between the Independent System Operator, the Scheduling Coordinator, and the Buildings offering Demand Response.}
    \label{fig:ISO_DR_Interactions}%\vspace{-0.3cm}
\end{figure}

